Does Face Recognition Accuracy Get Better With Age? Deep Face Matchers Say No

Previous studies generally agree that face recognition accuracy is higher for older persons than for younger persons. But most previous studies were before the wave of deep learning matchers, and most considered accuracy only in terms of the verification rate for genuine pairs. This paper investigates accuracy for age groups 16-29, 30-49 and 50-70, using three modern deep CNN matchers, and considers differences in the impostor and genuine distributions as well as verification rates and ROC curves. We find that accuracy is lower for older persons and higher for younger persons. In contrast, a pre deep learning matcher on the same dataset shows the traditional result of higher accuracy for older persons, although its overall accuracy is much lower than that of the deep learning matchers. Comparing the impostor and genuine distributions, we conclude that impostor scores have a larger effect than genuine scores in causing lower accuracy for the older age group. We also investigate the effects of training data across the age groups. Our results show that fine-tuning the deep CNN models on additional images of older persons actually lowers accuracy for the older age group. Also, we fine-tune and train from scratch two models using age-balanced training datasets, and these results also show lower accuracy for older age group. These results argue that the lower accuracy for the older age group is not due to imbalance in the original training data.

==> figures/age_balanced.tex <==
\begin{table*}[t]
    \small
    \setlength\tabcolsep{4pt}
    \centering
    \ra{1.1}
    \begin{tabular}{l|rrrr|rrrr|rrrr}
        \multicolumn{1}{l|}{}& \multicolumn{4}{c|}{\textbf{Whole Dataset}} & \multicolumn{4}{c|}{\textbf{African American Males}}& \multicolumn{4}{c}{\textbf{Caucasian Males}}\\
        \textbf{Matcher@Trainining subset} & \multicolumn{1}{c}{\textbf{Young}} & \multicolumn{1}{c}{\textbf{Middle}} & \multicolumn{1}{c}{\textbf{Old}} & \multicolumn{1}{c|}{\textbf{Diff.}} & \multicolumn{1}{c}{\textbf{Young}} & \multicolumn{1}{c}{\textbf{Middle}} & \multicolumn{1}{c}{\textbf{Old}} & \multicolumn{1}{c|}{\textbf{Diff.}} & \multicolumn{1}{c}{\textbf{Young}} & \multicolumn{1}{c}{\textbf{Middle}} & \multicolumn{1}{c}{\textbf{Old}} & \multicolumn{1}{c}{\textbf{Diff.}} \\ \hline
        VGGFace2@MSM1V2\_Young & 89.71& 81.97 & 74.64& 15.07 & 92.05& 85.62 & 80.67& 11.38 & 90.98& 84.13 & 73.74& 17.24\\
        VGGFace2@MSM1V2\_Middle& \textbf{91.15} & \textbf{87.39}& \textbf{81.3}& \textbf{9.85} & \textbf{93}& \textbf{90.08}& \textbf{85.45} & 7.55& \textbf{91.43} & 86.81 & 74.97& 16.46\\
        VGGFace2@MSM1V2\_Old & 89.14& 84.77 & 76.88& 12.26 & 90.69& 87.3& 83.42& \textbf{7.27} & 88.91& \textbf{87.35}& \textbf{84.66} & \textbf{4.25}\\ \hline
        ArcFace@VGGFace2\_Young& 95.98& 95.13 & 87.83& 8.15& 96.92& 95.99 & 92.76& 4.16& 95.87& 95.82 & 82.86& 13.01\\
        ArcFace@VGGFace2\_Middle & 95.65& 94.89 & 87.83& 7.82& 96.7 & 95.9& 93.7 & 3 & 95.53& 95.8& 86.73& 8.8\\
        ArcFace@VGGFace2\_Old& \textbf{98.05} & \textbf{97.23}& \textbf{94.34} & \textbf{3.71} & \textbf{98.44} & \textbf{97.86}& \textbf{97.86} & \textbf{0.58} & \textbf{96.99} & \textbf{97.66}& \textbf{94.51} & \textbf{2.48} 
    \end{tabular}
    \caption{True positive rates (\%) with a false match rate of $10^{-4}$ for VGGFace2 and ArcFace fine-tuned with different age group subsets with the difference between the best and worst group.} 
    \label{tab:fine_tuning}
    \vspace{-1em}
\end{table*}

==> figures/average_time_figure_new.tex <==
\begin{figure}[t]
    %\captionsetup{justification=centering}
    \centering
    \begin{subfigure}[b]{0.75\columnwidth}
        \centering
            \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/facenet/avg_time_score_aut_facenet_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/facenet/avg_time_score_imp_facenet_morph.png}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\columnwidth}
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/resnet/avg_time_score_aut_resnet_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/resnet/avg_time_score_imp_resnet_morph.png}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\columnwidth}
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/arcface/avg_time_score_aut_arcface_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.49\columnwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/arcface/avg_time_score_imp_arcface_morph.png}
        \end{subfigure}
    \end{subfigure}
    \caption{Match scores with increasing elapsed time between authentic (left) and impostors (right) pairs on the whole dataset for Facenet (top), VGGFace2 (middle) and ArcFace (bottom).}
    \vspace{-1em}
    \label{fig:avg}
\end{figure}

==> figures/average_time_figure_old.tex <==
\begin{figure*}[t]
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/facenet/avg_time_score_aut_facenet_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/facenet/avg_time_score_imp_facenet_morph.png}
        \end{subfigure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/resnet/avg_time_score_aut_resnet_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/resnet/avg_time_score_imp_resnet_morph.png}
        \end{subfigure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/arcface/avg_time_score_aut_arcface_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/arcface/avg_time_score_imp_arcface_morph.png}
        \end{subfigure}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/facenet/avg_time_score_aut_facenet_aa_male_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/facenet/avg_time_score_imp_facenet_aa_male_morph.png}
        \end{subfigure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/resnet/avg_time_score_aut_resnet_aa_male_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/resnet/avg_time_score_imp_resnet_aa_male_morph.png}
        \end{subfigure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/arcface/avg_time_score_aut_arcface_aa_male_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/arcface/avg_time_score_imp_arcface_aa_male_morph.png}
        \end{subfigure}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/facenet/avg_time_score_aut_facenet_c_male_morph.png}
            \renewcommand\thesubfigure{\alph{subfigure}1}
            \vspace{-1em}
            \caption{Authentic}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/facenet/avg_time_score_imp_facenet_c_male_morph.png}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \vspace{-1em}
            \caption{Impostor}
            \vspace{-0.5em}
        \end{subfigure}
        \addtocounter{subfigure}{-1}
        \caption{Facenet}
        \vspace{-0.5em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/resnet/avg_time_score_aut_resnet_c_male_morph.png}
            \renewcommand\thesubfigure{\alph{subfigure}1}
            \vspace{-1em}
            \caption{Authentic}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/resnet/avg_time_score_imp_resnet_c_male_morph.png}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \vspace{-1em}
            \caption{Impostor}
            \vspace{-0.5em}
        \end{subfigure}
        \addtocounter{subfigure}{-1}
        \caption{VGGFace2}
        \vspace{-0.5em}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/arcface/avg_time_score_aut_arcface_c_male_morph.png}
            \renewcommand\thesubfigure{\alph{subfigure}1}
            \vspace{-1em}
            \caption{Authentic}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.485\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/arcface/avg_time_score_imp_arcface_c_male_morph.png}
            \addtocounter{subfigure}{-1}
            \renewcommand\thesubfigure{\alph{subfigure}2}
            \vspace{-1em}
            \caption{Impostor}
            \vspace{-0.5em}
        \end{subfigure}
        \addtocounter{subfigure}{-1}
        \caption{ArcFace}
        \vspace{-0.5em}
    \end{subfigure}
    \caption{Match scores with increasing elapsed time between authentic (A) and impostors (I) pairs for whole dataset (top), African American males (middle), and Caucasian males (bottom).}
    \label{fig:avg}
    \vspace{-1em}
\end{figure*}

==> figures/average_time_figure_old1.tex <==
\begin{figure*}[t]
    \captionsetup{justification=centering}
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/facenet/avg_time_score_aut_facenet_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/resnet/avg_time_score_aut_resnet_morph.png}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/arcface/avg_time_score_aut_arcface_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/facenet/avg_time_score_imp_facenet_morph.png}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/resnet/avg_time_score_imp_resnet_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/arcface/avg_time_score_imp_arcface_morph.png}
        \end{subfigure}
    %\end{subfigure}
    
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/facenet/avg_time_score_aut_facenet_aa_male_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/resnet/avg_time_score_aut_resnet_aa_male_morph.png}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/arcface/avg_time_score_aut_arcface_aa_male_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/facenet/avg_time_score_imp_facenet_aa_male_morph.png}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/resnet/avg_time_score_imp_resnet_aa_male_morph.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/arcface/avg_time_score_imp_arcface_aa_male_morph.png}
        \end{subfigure}
    %\end{subfigure}
    
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/facenet/avg_time_score_aut_facenet_c_male_morph.png}
            \caption{Facenet \\ Authentic}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/resnet/avg_time_score_aut_resnet_c_male_morph.png}
            \caption{VGGFace2 \\ Impostor}
            \vspace{-0.5em}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/arcface/avg_time_score_aut_arcface_c_male_morph.png}
            \caption{ArcFace \\ Authentic}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/facenet/avg_time_score_imp_facenet_c_male_morph.png}
            \caption{Facenet \\ Impostor}
            \vspace{-0.5em}
        \end{subfigure}
    %\end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.32\textwidth}
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/resnet/avg_time_score_imp_resnet_c_male_morph.png}
            \caption{VGGFace2 \\ Impostor}
            \vspace{-0.5em}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{.159\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/arcface/avg_time_score_imp_arcface_c_male_morph.png}
            \caption{ArcFace \\ Impostor}
            \vspace{-0.5em}
        \end{subfigure}
    %\end{subfigure}
    \captionsetup{justification=raggedright}
    \caption{Match scores with increasing elapsed time between authentic and impostors pairs for whole dataset (top), African American males (middle), and Caucasian males (bottom).}
    \vspace{-1em}
    \label{fig:avg}
\end{figure*}

==> figures/dataset_average_images.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.8\columnwidth}
      \centering
      \begin{subfigure}[b]{.29\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/average_faces/male_c_young_group_average_image.png}
        \caption{Young}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.29\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/average_faces/male_c_middle_group_average_image.png}
        \caption{Middle}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.29\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/average_faces/male_c_old_group_average_image.png}
        \caption{Old}
      \end{subfigure}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[b]{0.8\columnwidth}
      \centering
      \begin{subfigure}[b]{.29\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/average_faces/male_aa_young_group_average_image.png}
        \caption{Young}
        \vspace{-0.5em}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.29\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/average_faces/male_aa_middle_group_average_image.png}
        \caption{Middle}
        \vspace{-0.5em}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.29\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/average_faces/male_aa_old_group_average_image.png}
        \caption{Old}
        \vspace{-0.5em}
      \end{subfigure}
      %\vspace{1em}
  \end{subfigure}
  \caption{Average face for Caucasian males (top) and African American males (bottom) age groups.}
  \label{fig:mean_faces}
  \vspace{-1em}
\end{figure}

==> figures/dataset_table_old.tex <==
\begin{table*}[t]
    \setlength\tabcolsep{5pt}
    \centering
    \ra{1.2}
    \begin{tabular}{l|rrr|rrr|rrr}
                           & \multicolumn{3}{c|}{\textbf{Whole Dataset}}                                         & \multicolumn{3}{c|}{\textbf{African American Male}}                                 & \multicolumn{3}{c}{\textbf{Caucasian Male}}                                       \\ 
                           & \multicolumn{1}{c}{Young} & \multicolumn{1}{c}{Middle} & \multicolumn{1}{c|}{Old} & \multicolumn{1}{c}{Young} & \multicolumn{1}{c}{Middle} & \multicolumn{1}{c|}{Old} & \multicolumn{1}{c}{Young} & \multicolumn{1}{c}{Middle} & \multicolumn{1}{c}{Old} \\ \hline
        \textbf{\# Subjects w/ only 1 image (removed)} & 457 & 428 & 151 & 271 & 271 & 98 & 98 & 92 & 35\\ 
        \textbf{\# Subjects} & 5,778 & 6,532 & 1,074 & 4,085 & 4,235 & 726 & 833 & 1,140 & 221\\
        \textbf{\# Images} & 21,665 & 25,604 & 3,622 & 16,799 & 16,891 & 2,387 & 2,690 & 4,140 & 837
    \end{tabular}
    \caption{Division of age groups.}
    \label{tab:dataset_groups}
    \vspace{-1em}
\end{table*}

==> figures/fmr_fnmr_figure.tex <==
\begin{figure*}[t]
    %\begin{subfigure}[b]{1\textwidth}
        \begin{subfigure}[b]{0.327\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/facenet/fmr_fnmr_facenet_morph1.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{0.327\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/facenet/fmr_fnmr_facenet_male_aa_morph1.png}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{0.327\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/facenet/fmr_fnmr_facenet_male_c_morph1.png}
        \end{subfigure}
    %\end{subfigure}
    \hfill 
    %\begin{subfigure}[b]{1\textwidth}
        \begin{subfigure}[b]{0.327\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/whole_group/resnet/fmr_fnmr_resnet_morph1.png}
            \caption{Whole dataset}
            \label{fig:fmr_fnmr_resnet_whole_group}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{0.327\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_aa/resnet/fmr_fnmr_resnet_male_aa_morph1.png}
            \caption{African American males}
            \label{fig:fig:fmr_fnmr_resnet_male_aa}
        \end{subfigure}
        \hfill 
        \begin{subfigure}[b]{0.327\textwidth}
            \centering
            \includegraphics[width=1\columnwidth]{images/MORPH/male_c/resnet/fmr_fnmr_resnet_male_c_morph1.png}
            \caption{Caucasian males}
            \label{fig:fig:fmr_fnmr_resnet_male_c}
        \end{subfigure}
        %\label{fig:fmr_fnmr_resnet}
    %\end{subfigure}
    \caption{FMR and FNMR curves for FaceNet (top), and VGGFace2 (bottom).}
    \label{fig:fmr_fnmr}
\end{figure*}

==> figures/impostor_samples.tex <==
\begin{figure*}[t]
    \begin{subfigure}[b]{1\linewidth}
      \begin{subfigure}[b]{.265\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/impostor_samples/male_c_young.pdf}
        \caption{19 and 29 (0.09)}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.265\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/impostor_samples/male_c_middle.pdf}
        \caption{35 and 45 (0.08)}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.265\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/impostor_samples/male_c_old.pdf}
        \caption{57 and 67 (\textbf{0.156})}
      \end{subfigure}
      \vspace{1em}
  \end{subfigure}
  \begin{subfigure}[b]{1\linewidth}
      \begin{subfigure}[b]{.265\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/impostor_samples/male_aa_young.pdf}
        \caption{19 and 29 (0.192)}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.265\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/impostor_samples/male_aa_middle.pdf}
        \caption{37 and 47 (0.208)}
      \end{subfigure}
      \hfill %%
      \begin{subfigure}[b]{.265\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/MORPH/impostor_samples/male_aa_old.pdf}
        \caption{53 and 63 (\textbf{0.289})}
      \end{subfigure}
  \end{subfigure}
  \caption{Examples of average-scoring (FaceNet) impostor pairs for Caucasian males (a)(b)(c) and African American males (d)(e)(f) with 10 years of age difference for the three age groups used: young (a)(d); middle (b)(e); and old (c)(f).}
  \label{fig:imp_examples}
\end{figure*}

==> figures/lbp_table.tex <==
\begin{table}[]
    \centering
    \scriptsize
    \setlength\tabcolsep{3pt}
    \begin{tabular}{l|rrr|rrr|rrr}
     & \multicolumn{3}{c|}{\textbf{Whole Dataset}}& \multicolumn{3}{c|}{\textbf{African American Males}} & \multicolumn{3}{c}{\textbf{Caucasian Males}} \\
     & \multicolumn{1}{c}{\textbf{Young}} & \multicolumn{1}{c}{\textbf{Middle}} & \multicolumn{1}{c|}{\textbf{Old}} & \multicolumn{1}{c}{\textbf{Young}} & \multicolumn{1}{c}{\textbf{Middle}} & \multicolumn{1}{c|}{\textbf{Old}} & \multicolumn{1}{c}{\textbf{Young}} & \multicolumn{1}{c}{\textbf{Middle}} & \multicolumn{1}{c}{\textbf{Old}} \\ \hline
    $10^{-5}$ && & && & && &\\
    $10^{-4}$ && & && & && &\\
    $10^{-3}$ && & && & && & 
    \end{tabular}
    \caption{LBP verification rate (\%) results.}
    \label{tab:lbp}
\end{table}

==> figures/related_work_table.tex <==
\begin{table*}[t]
 \setlength\tabcolsep{2pt}
 \footnotesize
 \centering
    \begin{tabular}{l|ccccccccc}
    \textbf{Work} & \textbf{\begin{tabular}[c]{@{}c@{}}Verification \\ Rates or ROC\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Authentic\\ Distribution\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Impostor\\ Distribution\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Age \\ Groups\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Ages on \\ Race/Gender\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Authentic Pairs\\ Elapsed Time\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Impostor Pairs\\ Age Difference\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Public\\ Dataset\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Public \\ Matchers\end{tabular}} \\ \hline
    Beveridge et al. \cite{Beveridge2009} & Yes & No & No & No & No & No & No & Yes & No \\
    Klare et al. \cite{Klare2012} & Yes & No & No & Yes & No & No & No & No & No \\
    Best-Rowden and K. Jain \cite{longitudinal_c} & Yes & No & No & No & Yes & Yes & No & No & No \\
    Best-Rowden and K. Jain \cite{longitudinal_j} & Yes & Yes & No & No & Yes & Yes & No & No & No \\
    Lu et al. \cite{Lu2018} & Yes & No & No & Yes & No & No & No & Yes & Yes \\
    Cook et al. \cite{cook2018} & Yes & No & No & Yes & Yes & No & No & No & No \\
    This work & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes 
    \end{tabular}
    \caption{Related work methodology summary.}
    \label{tab:related_work_table}
\end{table*}
